LightRidge: An End-to-end Agile Design Framework for Diffractive Optical Neural Networks

To lower the barrier to diffractive optical neural networks (DONNs) design, exploration, and deployment, we propose LightRidge, the first end-to-end optical ML compilation framework, which consists of (1) precise and differentiable optical physics kernels that enable complete explorations of DONNs architectures, (2) optical physics computation kernel acceleration that significantly reduces the runtime cost in training, emulation, and deployment of DONNs, and (3) versatile and flexible optical system modeling and user-friendly domain-specific-language (DSL). As a result, LightRidge framework enables efficient end-to-end design and deployment of DONNs, and significantly reduces the efforts for programming, hardware-software codesign, and chip integration. Our results are experimentally conducted with physical optical systems, where we demonstrate: (1) the optical physics kernels precisely correlated to low-level physics and systems, (2) significant speedups in runtime with physics-aware emulation workloads compared to the state-of-the-art commercial system, (3) effective architectural design space exploration verified by the hardware prototype and on-chip integration case study, and (4) novel DONN design principles including successful demonstrations of advanced image classification and image segmentation task using DONNs architecture and topology.

==> ae.tex <==
% LaTeX template for Artifact Evaluation V20201122
%
% Prepared by 
% * Grigori Fursin (cTuning foundation, France) 2014-2020
% * Bruce Childers (University of Pittsburgh, USA) 2014
%
% See examples of this Artifact Appendix in
%  * SC'17 paper: https://dl.acm.org/citation.cfm?id=3126948
%  * CGO'17 paper: https://www.cl.cam.ac.uk/~sa614/papers/Software-Prefetching-CGO2017.pdf
%  * ACM ReQuEST-ASPLOS'18 paper: https://dl.acm.org/citation.cfm?doid=3229762.3229763
%
% (C)opyright 2014-2020
%
% CC BY 4.0 license
%

%\documentclass{sigplanconf}

%\usepackage{hyperref}

%\begin{document}

%\special{papersize=8.5in,11in}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper, 
% please remove above part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

LightRidge is an open-source framework for end-to-end optical machine learning (ML) compilation, which connects physics to system. This framework provides user-friendly DSL to design, explore and deploy the DONN system with customization. To use the framework, the implemented computation kernels are enclosed within a Python package with easy installation of \textit{pip install lightridge}. Two execution files for raw DONN emulation and the hardware-aware codesign DONN emulation are provided in \textit{tutorial\_01\_raw.py} and \textit{tutorial\_01\_codesign.py}, respectively. We also provide the bash script \textit{run.sh} for the exploration flow including model training, model inference, and model visualization (See \href{https://github.com/lightridge/lightridge/tree/main/ASPLOS2024_AE}{Python tutorial}). Furthermore, we provide Colab tutorial for easy interactive training and visualization access (See \href{https://drive.google.com/file/d/1DVzvvei0GBXX_jZewNtusR7xLCA-TwDM/view?usp=sharing}{Google Colab Access}.). 


\subsection{Artifact check-list (meta-information)}

 

{\small
\begin{itemize}
  %\item {\bf Algorithm: }
  \item {\bf Program:} \texttt{Python}
  \item {\bf Model: } Diffraction optical neural networks.
  \item {\bf Data set:} Public data included in examples. Dataloaders are provided to elaborate additional datasets.
  \item {\bf Run-time environment:} Ubuntu 18 or above, macOS 10.15 (Catalina) or above, and RHEL.
  \item {\bf Hardware: } Minimum 256 GB storage, 64 GB memory, with CPU and GPU and compatible driver/library.
 % \item {\bf Run-time state: }
  %\item {\bf Execution: }
  %\item {\bf Metrics: } Prediction 
  \item {\bf Output: } Diffractive optical neural network numerical models, performance metrics, and visualization.
  \item {\bf Experiments: } The training, inference, and visualization of the 5-layer DONN system for the image classification task with MNIST10~\cite{lecun1998mnist} dataset. 
  \item {\bf How much time is needed to prepare workflow (approximately)?: } Less than 10 min.
 % \item {\bf How much time is needed to complete experiments (approximately)?: } 5 mins for tutorial examples.
  \item {\bf Publicly available?: } Yes. ''\texttt{pip install lightridge}'', and Google Colab Tutorials available.
  \item {\bf Code licenses: } GNU GPL 3.0
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}

LightRidge is packaged and publicly released at The Python Package Index (PyPI). The package is available to access and install by \texttt{pip install lightridge}.

\begin{itemize}
    \item Colab tutorial:  \href{https://drive.google.com/file/d/1DVzvvei0GBXX_jZewNtusR7xLCA-TwDM/view?usp=sharing}{Google Colab Access}. 
    \item Bash/Python scription tutorials: \url{https://github.com/lightridge/lightridge/tree/main/ASPLOS2024_AE}
    \item Visit LightRidge website at \url{https://lightridge.github.io/lightridge} for additional tutorials and documentations of the infrastructure. \href{https://lightridge.github.io/lightridge/lightridge_tutorial_ASPLOS24_AE.html}{Access the specific AE page}.
\end{itemize}




%{\em Obligatory}

\subsubsection{Hardware dependencies}

The accuracy performance can vary on different GPU versions with limited training efforts for demonstration. However, when trained with enough training efforts, e.g., enough training epochs, the difference between different hardware platforms is negligible. 

We provide two platforms for demonstration:

\begin{itemize}
    \item \textbf{Colab} for easy access and demonstration -- This tutorial is deployed on the T4 GPU of Colab, which is the default GPU as free GPU resources. In case of fast and feasible runtime in Colab, we reduce the training efforts to only 5 epochs for the raw DONN emulation and 3 epochs for the codesign DONN emulation, which results in degraded performance in Colab tutorial compared with the claimed performance in the paper. \href{https://drive.google.com/file/d/1DVzvvei0GBXX_jZewNtusR7xLCA-TwDM/view?usp=sharing}{Google Colab Access}.
    
    \item \textbf{Python Scripts} deployed on the server with dedicated Nvidia GPU (CUDA$\geq$11.x) -- These python files are implemented for command run on the server. Our implementations have been evaluated with 2080 Ti, 3090, and 4090 GPUs, with Intel Xeon(R) Gold 6230 CPU.
\end{itemize}

\subsubsection{Data sets}

We provide MNIST10~\cite{lecun1998mnist} dataset for demonstration. We also provide the parameter in the code to download FashionMNIST~\cite{xiao2017fashion} for image classification task. Moreover, we provide customizable dataloader in \texttt{lr.utils} for loading your own datasets.

\subsubsection{Models}

In this tutorial, we configure the model as a 5-layer DONN model with the same system setups shown in Section \ref{sec:validation} for demonstration. We provide both pre-configured basic DONN models in the python package in \texttt{lr.models} and the customized model construction demonstration in the main execution python file. Both are constructing a sequentially stacked 5-layer DONN systems for demonstration.

Following our comments in the Colab tutorial, you will be able to configure the optical neural architecture by modifying the parameters such as:

\begin{itemize}
        \item Laser source information: \texttt{wavelength} (default: 532e-9 in meter)
        \item System resolution/size: \texttt{sys\_size} (200)
        \item Pixel dimension: \texttt{pixel\_size} (3.6e-5 in meter)
        %\item Padding size for emulations: \texttt{pad} (100) 
        \item Mathematical approximation for light diffraction: \texttt{approx}
        \item Diffraction distance: \texttt{distance} (default: 0.3 in meter).
        \item System depth: \texttt{num\_layers} (default: 5)
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

Released as Packaged Python Project \texttt{lightridge}: \texttt{pip install lightridge}. Other two main execution files \textit{tutorial\_01\_raw.py} and \textit{tutorial\_02\_codesign.py}, and a bash script \textit{run.sh} are included in the folder.


 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

We provide two approaches for the demonstration:
\begin{itemize}
    \item For Colab tutorial, the code block is run one by one for interactive results feedback.

    \item For the python files, the execution flow for model training, inference, and visualization is implemented in \textit{run.sh}.
\end{itemize}

\noindent
The detailed experimental pipeline are organized as follows:

\begin{itemize}
    \item Step 1: LightRidge installation
    \item Step 2: Check LightRidge installation
    \item Step 3: Load packages and configure training devices
    \item Step 4: Constructing DONNs
    \item Step 5: Training DONNs
    \item Step 6: Visualization
    \item Step 7: Change the DONN model with codesign information
    \item Step 8: Add the device parameters
    \item Step 9: Visualization
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

Expected results should match \url{https://github.com/lightridge/lightridge/tree/main/ASPLOS2024_AE} and \href{https://lightridge.github.io/lightridge/lightridge_tutorial_ASPLOS24_AE.html}{Access the specific AE page}, in 1) accuracy metrics and 2) propagation and phase visualization.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment customization}

This framework provides customization for both model constructions and training setups. Different model constructions involve exploration efforts to find the paired parameters as shown in Section~\ref{sec:archtecture_variation}. The training setups such as learning rate (\textit{--lr}), training epochs (\textit{--epochs}), batch size (\textit{--batch\_size}), etc., can be customized by the arguments implemented in the python file. 

 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper, 
% please remove below part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\end{document}


==> compiler-table.tex <==
\begin{table*}[h]
\small
    \centering
      \caption{Overview of the LightRidge programming modules and partial front-end APIs. Note that we use \texttt{lr} to represent our integrated Python package \texttt{lightridge}.}
    \label{tab:language}
\begin{tabular}{|p{5em}|p{11em}|p{42em}|}

     \midrule
     Classes & Modular Programs & Description\\
     \midrule
     
     \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\\ \\ \\ ~~Low-level \\ ~~~modeling\end{tabular}} & Laser source \& profiles & Modeling coherent laser beams with various wavelength/profiles, e.g., Gaussian beam, Bessel beam, etc. \\
     
     \cmidrule(r){2-3}
     
     & Diffraction approximation & High-performance tensor implementations of numerical diffraction approximations, including \textbf{Rayleigh-Sommerfeld} (Equation \ref{equ:sommerfeld}), \textbf{Fresnel} (Equation \ref{equ:fresnel}), and \textbf{Fraunhofer} (Equation \ref{equ:fraunhofer}).  \\
     \cmidrule(r){2-3}
     
     & Optical/photon detector & An photon detector to capture the light intensity and convert the analog intensity information to the digital computer-processable information. \\
     \midrule
 
     \multirow{4}{*}{ \begin{tabular}[c]{@{}c@{}} \\ \\ \\ Model-level\\ APIs\end{tabular}} & \texttt{lr.laser} & Define the laser source for the system, including laser wavelenghth and its beam profile. \\
     \cmidrule(r){2-3}
    & \vspace{1mm}\texttt{lr.layers} & Include modules of different types of diffraction modeling, e.g., hardware-specific layer module \texttt{lr.layers.diffractlayer} and general diffractive layer \texttt{lr.layers.diffractlayer\_raw}, that can be configured with various approximation methods, distance, diffraction unit size, etc. \\
    \cmidrule(r){2-3}
    & \texttt{lr.layers.detector} & Define detector designs for various ML tasks, e.g., in image classification task, the coordinate and the size of the detection region for each candidate class. \\
    \cmidrule(r){2-3}
    & \texttt{lr.models} & Sequential container to customize DONN system by stacking diffractive layer and detector modules.\\
     \midrule
     
     
     \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} \\  ~~~Training \end{tabular}} &  \vspace{0.2mm}\texttt{lr.train.utils} & Training utility modules including data handling (e.g., \texttt{utils.data\_to\_cplex}), complex-valued regularization, loss function, optimizer, etc.\\
     \cmidrule(r){2-3}
         & \texttt{lr.train.to(device)} & Enable CPU and GPU accelerations for accelerating diffraction emulation and DONNs training.  \\ \cmidrule(r){2-3}
          & \texttt{lr.train.dse(specs)} & Perform pre-fabrication design space exploration with chip integration specifications as inputs.   \\
        % \cmidrule(r){2-3}
        % & \texttt{lr.traioptimizer} & Visualization of emulated propagation process through the system. \\
        \midrule
    \multirow{2}{*}{\begin{tabular}[|c|]{@{}c@{}}  Hardware \\ deployment\end{tabular}}  & \texttt{lr.layers.view()} & Visualize the original phase value per layer or values w.r.t the hardware specifications. \\
    \cmidrule(r){2-3}
    
    &\texttt{lr.model.to\_system} &  Generate device-specific phase parameters for deployment w.r.t the hardware specifications (e.g., configurations of SLMs, thickness of 3D printed masks). \\
     \midrule
\end{tabular}
  %\vspace{-3mm}
\end{table*}


\iffalse
\begin{table*}[]
\small
    \centering
    \begin{tabularx}{\linewidth}{  
    | >{\raggedright\arraybackslash}p{5em} 
    | >{\raggedright\arraybackslash}p{16em}
    | >{\raggedright\arraybackslash}X |}
    \hline
         class & Modular Prog. & Description\\
         \hline
         \multirow{3}{*}{\begin{tabular}[|c|]{@{}c@{}}lower-level \\ module\end{tabular}} & \texttt{lr.laser} & Define the laser source for the system, including laser wavelenghth and it profile, e.g., Gaussian beam, Bessel beam, etc. \\
         \cmidrule(r){2-3}
         & \texttt{\texttt{lr.layers.DiffractLayer}} & Define the detailed diffraction information in the system, including the size information of diffractive layers, the diffraction approximation methods, the diffraction distance between layers, etc. \\
         \cmidrule(r){2-3}
         & \texttt{lr.layers.Detector} & Define the pre-defined detector regions for each class on the detector plane, including the coordinate information and the size of the detector region for each class. \\
         \hline
         DONN Model & \texttt{Class Model(): ...} & Customize the DONN system by stacking defined diffractive layers and detector plane in arbitrary ways.\\
         \hline
         \multirow{3}{*}{high-level module} & \texttt{train(model, device, ...)} & Call the training function where dataset, optimizer, loss function, learning rate, etc are defined.\\
         \hline
         & \texttt{model.phase\_view()} & Visualization of phase modulation in each diffractive layer. \\
         \hline
         & \texttt{model.prop\_view()} & Visualization of emulated propagation process through the system. \\
         \hline
         Hardware deployment & \texttt{model.to\_slm() model.to\_3d\_render()} & Provide interface with hardware backends. \\
         \hline
         
    \end{tabularx}
    \caption{{Illustration for the modular program block in the compiler. We first import \texttt{LightRidge} as \texttt{lr}.}
    \label{tab:language}}
\end{table*}
\fi

==> figs/dse_figures.tex <==

\begin{figure*}[t]
     \centering
 
      \begin{subfigure}[b]{0.235\textwidth}
         \centering
    \includegraphics[width=1\textwidth]{isca2022-latex-template/figs/micro22_runtime/runtime_lightridge_cpu-crop.pdf}
         \caption{LightRidge-CPU results.}
        \label{fig:runtime_2}
     \end{subfigure}
    \begin{subfigure}[b]{0.235\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{isca2022-latex-template/figs/micro22_runtime/runtime_lightridge_gpu-crop.pdf}
         \caption{LightRidge-GPU results.}
         \label{fig:runtime_44}
     \end{subfigure}
     \begin{subfigure}[b]{0.235\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{isca2022-latex-template/figs/micro22_runtime/runtime_lightpipe-crop.pdf}
         \caption{LightPipe(2021) results.}
         \label{fig:runtime_1}
     \end{subfigure}
     \begin{subfigure}[b]{0.235\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{isca2022-latex-template/figs/micro22_runtime/cpu_speedups-crop.pdf}
         \caption{CPU speedups.}
         \label{fig:runtime_0}
     \end{subfigure}
     \caption{Runtime evaluation of LightRidge with various workloads of emulating DONNs systems that are configured in different system dimension sizes ($N$) and depths ($D$) -- \textbf{(a)} runtime results collected with LightRidge CPU execution, \textbf{(b)} LightRidge GPU execution, \textbf{(c)} up-to-date LightPipe(2021), and \textbf{(d)} CPU speedups results over LightPipe(2021).}
     \label{fig:runtime}
    % \vspace{-5mm}
\end{figure*}


==> isca2022-latex-template/01sec-intro_old.tex <==
\section{Introduction}\label{sec:intro}
\vspace{3mm}

During the past half-decade, there has been significant growth in machine learning with deep neural networks (DNNs). DNNs improve production in many areas like large-scale computer vision, natural language processing (NLP), and data mining tasks \cite{lecun2015deep}. DNNs designed for different applications can vary significantly from each other in the system structure, e.g., DNN systems designed for NLP such as LSTM, usually have large memory accesses but less average computation on fetched data, which means such DNN systems are memory-bounded \cite{han2017ese}. While DNN systems designed for image classification such as convolution neural networks will have less memory access but more average computations on each single fetched data, i.e., such DNNs are computation-bounded \cite{dean20201}. As a result, platforms designed for general purposes (e.g., CPUs) may not realize the best performance for various DNN applications. Thus, specialized DNN accelerators and domain-specific compilation become the best meaning for DNN accelerations to satisfy the performance requirements in broad application scenarios \cite{nvidia2017v100,chen2016eyeriss,jouppi2018domain,lai2019heterocl,zhang2018dnnbuilder,sharma2018bit,tambe2021edgebert}. 

Similar to most general-purpose and specialized computing platforms, there is an obvious trade-off in between the performance of computing and resource and power efficiency. While there have recently seen great progress in customized accelerators that adjust the computing performance with efficiency in hardware architectures and systems, the Pareto-frontier of conventional accelerators are remaining the same \cite{dean20201,lecun2015deep,ragan2013halide}. For example, for applications requiring high throughput in datacenter systems, high-performance accelerators such as \textit{Tensor Processing Unit} (TPU) \cite{jouppi2018domain} and \textit{Nervana} \cite{rao2018beyond} significantly increase the computing throughput, which simultaneously introduce very high power consumption. On the other side, embedded and emerging accelerators, which are designed for specific neural networks and accelerators implemented in the Internet of things (IoT) systems \cite{simon2019blade,cass2019taking,verhelst2017embedded,tambe2021edgebert,reagen2016minerva,wu2019machine}, focus on improving resource and power efficiency but offer limited functionality and throughput. 

To advance the Pareto-frontier of conventional DNN accelerators, i.e., offering high computing performance as well as extreme power efficiency, accelerators taking advantage of optics, namely \textit{optical neural networks} (ONNs), have recently attracted significant interests in machine learning and hardware acceleration. The main advantages of ONNs over conventional neural networks on digital platforms can be summarized as follows -- \textbf{(1)} DNN systems rely heavily on fixed matrix multiplications. In optical computing systems, since the input features are encoded and carried by light, the computation and data movement will happen at the light speed with orders of magnitude advantages in power consumption \cite{gu2020towards,shen2017deep,hamerly2019large,xu202111,gao2021artificial}. 
%For example, a common lens can perform a Fourier transform naturally by physics without power consumption and it can perform certain matrix operations optically without consuming power \cite{}.
{\textbf{(2)} The laser implemented in the optical systems can be easily expanded with passive optical devices, such as the beam splitter, to multiple channels, which means parallel computation can be easily realized with ONN systems and the throughput of the system will be significantly increased \cite{lin2018all,mengu2020scale,zhou2021large}. \textbf{(3)} The trained DONN system will be deployed with passive optical devices, which means there will no additional energy cost for inference process and improve the energy efficiency significantly \cite{shen2017deep,ying2020electronic,gu2020towards,feldmann2021parallel,li2021real}}.

%Once a neural network is trained, the optical devices implemented in the optical system are passive devices, which means there will be no additional energy cost for the inference process, highly improving the energy efficiency \cite{shen2017deep,ying2020electronic,gu2020towards,feldmann2021parallel}. }

%(1) They rely heavily on fixed matrix multiplications. Linear transformations (and certain non- linear transformations) can be performed at the speed of light and detected at rates exceeding 100 GHz (ref. 19) in photonic networks and, in some cases, with minimal power consumption20,21. For example, it is well known that a common lens performs a Fourier transform without any power consumption and that certain matrix operations can also be performed optically without consum- ing power. (2) They have weak requirements on nonlinearities. Indeed, many inherent optical nonlinearities can be directly used to implement nonlinear operations in ONNs. (3) Once a neural network is trained, the architecture can be passive, and computation on the optical signals will be performed without additional energy input.

Nowadays, two main trends of ONN systems have been explored and employed to accelerate deep learning systems. First, Shen et al., \cite{shen2017deep} proposed optical interference unit (OIU), which is employed to accelerate the matrix multiplication and attenuation in conventional neural networks. Specifically, such systems aim to accelerate conventional DNN algorithms by introducing optical arithmetic operators with extreme parallelization and power efficiency, as well as accelerating on-chip data movement \cite{ying2020electronic,shen2017deep,wang2018integrated}. {However, the Mach-Zehnder Interferometer (MZI) electro-optic modulators require accurate chip fabrication, and the small fabrication error in each unit accumulates as the light propagates in the MZI mesh. Both factors limit the scalability of matrix multiplication.} On the other hand, \textit{diffractive optical neural networks} (DONNs) mimic the propagation and connectivity properties of conventional neural networks by utilizing the diffraction of coherent light \cite{lin2018all,li2021real,mengu2020scale,zhou2021large}. Specifically, by taking advantage of the physical diffraction phenomenon, DONN systems will work similarly to fully connected neural networks but with extremely high neuron density, featuring millions of neurons in each layer interconnected with neurons in neighboring layers \cite{lin2018all}. More importantly, the propagation delay of each diffractive neural layer is constant regardless of the density of neurons, at the speed of light. In DONN systems, each pixel in the diffractive layers can be seen as a neuron in the fully connected neural network. At each pixel, the input light beam will be phase modulated and diffracted. Moreover, for hardware deployment, layers employed in DONN models are cheaper and easier to fabricate with a decent 3D printer compared to other photonic techniques \cite{shen2017deep}. In addition, \cite{lin2018all, rahman2021ensemble, li2021real} demonstrated that the diffractive propagation controlled by physical parameters in DONN systems is differentiable, which can be optimized with a conventional automatic differentiation engine.


However, the design of the DONN model from scratch can be a great challenge as building a DONN model requires fundamental domain-specific knowledge in optics, and high programming efforts for constructing, emulating and training the physical parameters of DONNs. %Existing  python  packages like LightPipe \cite{vdovin1997lightpipes} provide simple model simulation for coherent optical devices with essential diffraction. However, to build a DONN model, the diffraction between layers needs to be differentiated and cascaded to form a complete DONN. Moreover, the emulation of diffraction is most built for CPUs, which has an unsatisfactory exploration efficiency and waste the parallelism in the computation of DONN systems.  
Thus, we propose \textit{LightRidge}, an end-to-end compiler framework to greatly lower the barriers of design and exploration of DONN systems. In particular, \textit{LightRidge} simplifies the exploration for optical neural networks with \textbf{high-performance, precise, versatile, and differentiable optical physics kernels, which precisely correlate to experimental physical systems that enable first-ever out-of-box software-to-hardware realization in end-to-end fashion.} %Our framework enables effective training  %Three diffraction algorithms have been implemented in the compiler, i.e., Rayleigh-Sommerfeld, Fresnel, and Fraunhofer \cite{goodman2005introduction} and our experiments in Section \ref{sec:validation} have verified that the physical engines are accurate enough to be corresponding with the practical deployment, enabling complete explorations of diffractive optical neural networks. 
%\textbf{(2) High-performance physics emulation kernels optimized on CPUs and GPUs}, which offer orders of magnitude runtime improvements compared to existing state-of-the-art conventional optical emulators in training and emulation. \textbf{(3) Versatile optics ML modules enable flexible DONNs modeling and physics-aware architecture exploration}. \textbf{(4) First optical ML DSLs and physical hardware deployment integration} --
Our framework also provides a first-ever optical ML DSL to simplify design, explore, and deployment of DONNs in real-world scenarios, which will significantly reduce the engineering efforts to advance the research in optical neural networks. Specifically, for the backend deployment, our compiler provides end-to-end deployment all the way to optical devices or fabrication systems, e.g., in a TeraHertz (THz) system, the diffractive layers can be fabricated with 3D printers with specific materials \cite{lin2018all}, while in a visible range system, the diffractive layers can be realized with spatial light modulators (SLMs) \cite{zhou2021large}. 

\begin{table}[h]
  \caption{Overview comparisons of existing programming frameworks for DONNs compilation. Note that the Lines of Code (LoC) efforts are evaluated with a 5-layer DONNs \cite{lin2018all}. \fixme{correlation metric}}
  % \vspace{2mm}
  \label{table:compiler_comp}
  \centering
  \scriptsize
 %   \resizebox{0.98\columnwidth}{!}{%
  \begin{tabular}{c|c|c|c|c|c|c}
    \toprule
        &  \begin{tabular}[c]{@{}c@{}}Optics \\ kernels\end{tabular} & \begin{tabular}[c]{@{}c@{}}CPU \\ \end{tabular} & \begin{tabular}[c]{@{}c@{}}GPU \\ \end{tabular} & \begin{tabular}[c]{@{}c@{}}Batch \\ Ops\end{tabular}& \begin{tabular}[c]{@{}c@{}}LoC efforts \\ (inference)\end{tabular} & \begin{tabular}[c]{@{}c@{}}LoC efforts \\ (training)\end{tabular} \\
         \midrule
         LightRidge & \cmark & \cmark & \cmark & \cmark & 1 & 1\\
         \midrule         
         LightPipe\cite{vdovin1997lightpipes} & \cmark & \cmark &  \xmark & \xmark & 1.2$\times$ & n/a\\
         \midrule
         \begin{tabular}[c]{@{}c@{}}Customized\\ PyTorch/TF\end{tabular} & \xmark & \cmark & \cmark & \cmark & 20$\times$ & 50$\times$ \\
    \bottomrule
  \end{tabular}
%}
\end{table}
% old text - first isca submission
%However, the design of the DONN model from scratch can be a great challenge as building a DONN model requires fundamental domain-specific knowledge in optics, and high programming effort for constructing, emulating and training the physical parameters of DONNs. %Existing  python  packages like LightPipe \cite{vdovin1997lightpipes} provide simple model simulation for coherent optical devices with essential diffraction. However, to build a DONN model, the diffraction between layers needs to be differentiated and cascaded to form a complete DONN. Moreover, the emulation of diffraction is most built for CPUs, which has an unsatisfactory exploration efficiency and waste the parallelism in the computation of DONN systems.  
%Thus, we propose \textit{LightRidge}, an end-to-end compiler framework to greatly lower the barriers of design and exploration of DONN systems. In particular, \textit{LightRidge} simplifies the exploration for optical neural networks with \textbf{(1) precise, versatile, and differentiable optical physics kernels} -- Our compiler offers versatile physics modeling that precisely correlates to experimental physical systems and also takes advantage of conventional back-propagation optimization engines by enabling differentiability of the diffraction modeling. %Three diffraction algorithms have been implemented in the compiler, i.e., Rayleigh-Sommerfeld, Fresnel, and Fraunhofer \cite{goodman2005introduction} and our experiments in Section \ref{sec:validation} have verified that the physical engines are accurate enough to be corresponding with the practical deployment, enabling complete explorations of diffractive optical neural networks. 
%\textbf{(2) high-performance physics emulation kernels optimized on CPUs and GPUs.} -- LightRidge compiler provides high-performance training and inference capability for DONN systems by taking full advantage of modern computation platforms. \textbf{(3) versatile optics ML modules enable flexible DONNs modeling and architecture exploration} -- In the compiler, the mathematical computation and functions have been implemented, and different algorithms are provided for different application scenarios. Users can customize their model w.r.t arbitrary optical systems by simply stacking the parameterized layer modules. \textbf{(4) first optical ML DSLs and physical hardware deployment integration} -- To make our compiler accessible and extensible to users, we provide a simple DSL model in LightRidge to simplify design, explore, and deployment of DONNs in real-world scenarios. Specifically, for the backend deployment, our compiler provides end-to-end deployment all the way to optical devices or fabrication systems, e.g., in a TeraHertz (THz) system, the diffractive layers can be fabricated with 3D printers with specific materials \cite{lin2018all}, while in a visible range system, the diffractive layers can be realized with spatial light modulators (SLMs) \cite{zhou2021large}.
% After the simulation of DONN system with our compiler, by simply calling the code block, the required files for 3D printing will be generated automatically for users. 
%To make our compiler accessible and readable for users, we simplify users' parameter selections by providing both manual parameters inputs and automatic parameters optimizations. On the other hand, our compiler also provides supports for backend hardware deployment by generating the files needed for devices fabrications, e.g., in a TeraHertz (THz) system, the diffractive layers can be fabricated with 3D printers with specific materials. After the simulation of DONN system with our compiler, by simply calling the code block, the required files for 3D printing will be generated automatically for users. 
The contributions of this paper are summarized as follows:


\begin{itemize}
    \item We introduce the first optical ML compiler \textbf{LighRidge}, which consists of versatile optical physics modeling that enable efficient and precise DONNs modeling w.r.t to real-world optics system and its ML applications. 
    \item We address the miscorrelation limitations between numerical physics modeling and real-world optical hardware system, which enables seamless deployment from software emulation to hardware realization in out-of-box fashion.
    \item We experimentally verify the correlation between the numerical physics kernels using our physical optical systems in visible frequency range (Sections \ref{sec:validation} and \ref{sec:result_visible}), which do not require any manual calibration efforts \cite{lin2018all} or post-implementation adaptive training \cite{zhou2021large}.
    \item LightRidge introduces high-performance Fourier optics physics kernels with CPU and GPU acceleration supports, which improve the emulation computations of Fourier optics propagation up to 7,661$\times$ speedups over the state-of-the-art (SOTA) simulator LightPipe\footnote{LightPipe is also in commercial use \url{http://www.okotech.com/lightpipes}.} \cite{vdovin1997lightpipes} while emulating and training multi-layer DONNs.% accelerated with supported by CPU and GPU acceleration
    \item We propose a novel complex-valued regularization training technique by leveraging optical physics domain-knowledge to enable efficient exploration of DONNs architecture and training methodologies, which overcome the classification performance bottlenecks of few-layer ($\le$3) DONNs systems over SOTA studies by \cite{lin2018all, zhou2021large}.
    \item We provide efficient architectural exploration demonstrations of DONNs w.r.t image classification tasks, which offer critical domain-knowledge to optimize the DONNs hardware implementation.
    %\item We propose three approximation methods for the DONN physical modelling and verify the accuracy for the physical emulation engine by deploying on various practical systems in Section \ref{sec:validation}.
    %\item We integrate our work in an end-to-end compiler framework \textit{LightRidge}, which significantly simplifies the design, exploration, and deployment of the DONN, lowering the barrier to get more researchers involved in DONNs explorations. 
    %\item We evaluate the performance of \textit{LightRidge} by providing a case study in section \ref{sec:casestudy}, which shows great runtime improvements of more than \textbf{107$\times$} speedup. Also, the gap between numerical modelling and physical deployment is narrowed with our compiler.
    \item Finally, LightRidge DSL significantly simplifies the engineering efforts of design, exploration (Table \ref{table:compiler_comp}), and deployment of the DONNs, and lower the barriers of realizing DONNs systems\footnote{\color{blue}LightRidge compiler will be fully released as open-source at xxx. Tutorial example of reproducing 5-layer DONNs training and evaluation is included at \url{https://anonymous.4open.science/r/test-24C6/isca2022_lightridge_response.ipynb}}. %Specifically, we demonstrate the capabilities of LightRidge using three optical systems in different frequency range, and validate the deployment with complete visible range optical systems (Figures \ref{fig:prop_exp} and \ref{fig:prop_sim}).
\end{itemize}
 

==> isca2022-latex-template/02sec-background.tex <==
\section{Background}\label{sec:background}
 
\iffalse
\begin{figure}[!htb]
  \centering
  \includegraphics[width=1 \linewidth]{isca2022-latex-template/figs/comparison_ml_compiler-crop.pdf}
  \caption{Comparisons between conventional ML compilation stack with optical ML (DONNs in specific) compilation stack.}
  \label{figs:ml_compiler_compare}
\end{figure}
\fi



%Conventional ML compilation mostly consists of two stages -- 1) front-end ML compiler that offers building blocks for designing, training, and validating deep neural networks, and 2) back-end compiler with domain-specific hardware optimizations or hardware generation, supported with a high-level programming interface. The front-end ML compilation and back-end optimization are mostly decoupled. While front-end ML frameworks such as PyTorch \cite{paszke2019pytorch}, Tensorflow \cite{abadi2016tensorflow}, MXNet \cite{chen2015mxnet}, etc., that offer end-to-end compilation from designing and training to general purpose hardware deployment, real-world applications require more customized and optimized deployment for various platforms ranging from large-scale data centers to low-power edge systems. 
\noindent
\textbf{DL Compilation and Acceleration} -- Recently, there have significant progress in full-stack compilation framework with domain-specific hardware-software (HW-SW) codesign methodologies, which aims to produce Pareto-optimal hardware acceleration solutions by integrating the software level optimizations w.r.t specific hardware back-end characteristics \cite{chen2018tvm,lai2019heterocl,rotem2018glow,lattner2020mlir,zheng2020flextensor,sharma2018bit,sharma2016high,huang2021cosa}, mostly supported by well-developed digital hardware backend supports (e.g., CPU/GPU/FPGA). %For example, TVM \cite{chen2018tvm} compiles ML models with domain-specific runtime optimization on CPUs, GPUs, and ML accelerators; HeteroCL \cite{lai2019heterocl} and DNNBuilder \cite{zhang2018dnnbuilder} provides more specific optimization for FPGA backend, where the generated code is then compiled to FPGA implementation. As we can see, the ML compilation frameworks for conventional digital platforms are all connected to existing low-level compiler systems, e.g., LLVM \cite{lattner2004llvm} for CPU deployments, Xilinx Vivado for FPGAs compilation \cite{o2014xilinx}. In other words, optimizations in existing ML compilers are \textit{"optimizing behaviors of low-level compilers"}. 
In contrast, the deployment of DONN systems is performed directly on the fabrication-level or device-level, in which the compilation process of DONNs needs to bridge the high-level algorithms to low-level physics and devices.%, e.g., 3D printed mask \cite{lin2018all} or spatial light modulators (SLMs) \cite{zhou2021large}. 
%More importantly, there have been great challenges in precisely correlate numerical modeling of DONNs w.r.t to specific optics setups, due to the complex physics emulation and system noise. For example, Zhou et. al \cite{zhou2021large} reported 33\% accuracy gap between the numerical modeling versus their experimental measured accuracy in optical systems with wavelength in visible range. 
To minimize the miscorrelation gap, it generally requires significant manual engineering efforts to calibrate or adaptively train the DONNs system \cite{lin2018all,zhou2021large}. Our LightRidge compiler aims to precisely correlate the physical implementation with the numerical modeling (train and test), to enable out-of-box software-to-hardware deployment.


\iffalse
\subsection{Optical Neural Networks}
\label{sec:onn}
 
Recently, optical neural networks have been an emerging area for deep learning systems because of its great advantages in saving energy, computing in high speed, and easily realizing parallel computation. There are two directions for utilizing optical systems in dealing with deep learning tasks. The first direction is to use optics to accelerate the computation-density parts, such as matrix multiplication in conventional transistor-based digital platforms. For example, the optical interference unit (OIU) proposed by \cite{shen2017deep} enables input modification based on Mach-Zehnder Interferometers (MZI). Specifically, the input light beam will be coupled and decoupled in MZI such that two sub-beams will be applied with different phase modulation. Thanks to the interference happening in MZI, a configurable weights matrix will be introduced by phase modulation and the multiplication between weight matrix and input matrix will be realized by interference. In such an optical system application, the power consumption for each multiplication will be significantly reduced compared to the transistor-based platforms. However, small power is still required to maintain the phase modulator settings and needs to be fabricated with high precision \cite{shen2017deep}.

The second direction is to use all-optical neural networks to mimic fully connected neural networks. Specifically, the diffractive optical neural network (DONN) realizes neuron connection with light diffraction and phase modulation \cite{rahman2021ensemble,lin2018all,zhou2021large,li2021spectrally}. As shown in Figure \ref{fig:onn_full}(c), at each diffraction unit in the diffractive layers, the input light wave will be diffracted by the aperture of the unit. Meanwhile, with different phase modulation implemented at the diffraction unit, the input wave will be phase modulated simultaneously.%As a result, the input light wave will be phase-modulated at each diffraction unit and connected to all units at the neighboring layer by light diffraction. 
In DONN systems, we can easily expand the system size by re-fabricating the diffractive layers with larger sizes. Once the layers are trained and fabricated, they will be passive optical devices in the system and will function with no power consumption. Moreover, the fabrication of the trained diffractive layers can be easy and cost-efficient with a decent 3D printer, where the phase modulation is encoded with the thickness of the 3D printed material, or a configurable phase modulator such as SLM, where the provided phase modulation is controlled by the applied voltage to each diffraction unit (liquid crystal) in the SLM.
\fi

\noindent
\textbf{Hardware Deployment for DONNs} -- To deploy the trained DONN model on physical hardware, we need to select the optical devices carefully with the knowledge in materials, as optical devices made from different materials can have significantly different response to different laser wavelength. Specifically, optical devices functioning as diffractive layers is expected to provide light diffraction and around 2$\pi$ phase modulation in the DONN system, and the detector used to capture the light intensity at the end of the system is expected to show descent linear response to the light intensity under specific laser wavelength. For example, the Spatial Light Modulators (SLMs)\footnote{\small \url{https://holoeye.com/lc-2012-spatial-light-modulator/}} made with twisted nematic (TN) liquid crystal can provide a phase shift of about $2\pi$ at $450$nm, about $1.8\pi$ at $532$nm and around $1\pi$ at $800$nm w.r.t the full range of supplying control voltage, and it shows no response to other wavelength range. Thus, such SLMs can only function as diffractive layers in the DONN system with laser wavelength in visible range. For systems with laser wavelength in Terahertz (THz) range, i.e., $0.1$mm to $1$mm, a 3D printed mask with designed thickness at each pixel made with UV-curable resin can be used as the diffractive layers in THz optical systems \cite{lin2018all}.

%In our experimental hardware systems, the wavelength of the laser source is $532$nm, which is in the operating range of the SLM. Specifically, the SLM is an array of twisted nematic (TN) liquid crystal, which can be twisted to different angles by different applied control voltages, providing different phase modulation for the input light beam. Each pixel in the SLM is a liquid crystal independently controlled by the control voltage, which can be customized by users via HDMI. However, each single SLM can response differently even under identical experimental setups due to fabrication errors. When multiple SLMs are employed in one system, the error will accumulate, and worsening the correlation between the numerical emulations and the physical hardware experiments, which highlights the importance of the precise computation kernels for emulation and the hardware-software codesign algorithms designed specifically for DONN systems.  


%On one hand, HW-SW codesign focuses on optimizing the performance of low-precision DNNs models for inference acceleration. For example, \cite{zhang2018dnnbuilder} Quantization-aware training (QNNs IBM) 

%HeteroCL \cite{lai} xxx.

%Review hardware-software codesign methodologies in 1) HW-cost aware training in combined loss (e.g., DNNBuilder), 2) quantization-aware and noise resilient training (MXNet, QNN), 3) compilation aware optimization (primitives optimization; TVM HeteroCL). Emphasize on the differences in hardware deployment of the proposed compiler.



==> isca2022-latex-template/03sec-donn.tex <==
\section{Diffractive Neural Networks}\label{sec:donn}
 
This section presents the overview of DONNs, and the fundamentals of physical modeling, and theories for scalar light diffraction, which are critical elements to form multi-layer DONN systems for ML applications. {In a DONN system, diffractive layers are stacked in sequence. The information encoded light wave propagates, is phase-modulated, and diffracts at each diffractive layer. In accordance with the Huygens-Fresnel principle, each point at a given diffractive layer acts as a secondary source of the input light wave, the phase of which is determined by the product of the input wave and the complex-valued phase modulation at that point. The diffraction space is required to generate the diffraction pattern at the receive plane. The phase modulation at each point is the learnable parameter that is iteratively adjusted during the training process with error back-propagation method \cite{lin2018all, zhou2021large}. 
Note that the main physics kernels implemented in LightRidge aim to precisely and efficiently emulate the DONN system with the widely used approximation functions for scalar diffraction formulas discussed in this section.}
%implement all the approximation functions of widely used scalar diffraction formulas discussed in this section.}

\subsection{Overview of DONNs and Hardware Prototype}
\label{sec:implement_DONN}
 

As shown in Figure \ref{fig:onn_full}(a), the DONN system is majorly composed of three parts, i.e., the laser source, the diffractive layers and the detector. The continuous-wave (CW) laser source will encode the input information with the intensity of the light and the phase of the input wave will be initialized as $0$. The light wave and the phase modulation will be described with complex numbers in the system.

The detailed illustration of light propagation and phase modulation happening at each diffractive layer in the system is shown in Figure \ref{fig:onn_full}(c). Each diffractive layer is composed with dense diffraction units with apertures and phase modulator. Specifically, the aperture will provide light diffraction, which connects the neurons in neighboring diffractive layers. The phase modulation embedded in each aperture functions as weights in DONN to modify the input light wave, and the phase modulation is our targeted trainable parameters in the system. For the DONNs with different laser source, parameters for diffractive layers such as the size of diffraction unit, the distance between diffractive layers, and the materials used to fabricate diffractive layers can be totally different. 

%For the DONN with different laser source, parameters for diffractive layers such as the size of diffraction unit, the distance between diffractive layers, and the materials used to fabricate diffractive layers can be totally different. For example, for the DONN system with laser source with wavelength of $698nm$ (visible range), the diffraction units have the size of $7.6um \times 7.6um$, the distance between layers is $20cm$, and the diffractive layers are realized with SLMs \cite{zhou2021large}. However, for the DONN system with the laser source whose wavelength is $0.75mm$, the diffraction unit has the size of $0.4mm \times 0.4mm$, the distance between layers is $3cm$, and the diffractive layers are fabricated with {UV-curable resin} with a 3D printer \cite{lin2018all}.

The detector is used to capture the light intensity at the end of the system. We can generate the prediction results based on the intensity projected on the pre-defined region representing a specific label. For example, in a DONN system for image classification with MNIST10 dataset \cite{lecun1998mnist}, we define $10$ regions with size of $10 \times 10$ on the detector plane representing classes from $0 - 9$ (Figure \ref{fig:onn_full}(a)), if the region of class 1 has the highest average light intensity after propagation, the prediction result for the input with DONN will be class 1. 

While the DONN system is employed for ML tasks, such as image classification, phase parameters that modifies the layer-wise diffraction will be optimized through an iterative training process, just like conventional neural networks. With mathematical approximation shown in Section \ref{sec:fourier}, the DONN forward function is described in complex domain, and at numerical level is fully differentiable from detector to laser input. Therefore, the training process of DONNs in LightRidge can be fully integrated with existing automatic differentiation engines and stochastic gradient descent optimization algorithms. To initialize the training process, DONNs w.r.t ML tasks will have a loss function calculated based on the prediction of the model. Uniquely, DONNs predictions are generated by measuring the output intensity at customized detector regions, which mimics the probabilities of output prediction after \texttt{softmax} in conventional DNNs. %{ non-linearity discussion.} %For example, mean square error loss (\texttt{MSELoss}) is used in our implementation to guide the training process of DONNs, which is iteratively optimized with training parameters such as training epochs, learning rate, learning rate decaying, etc.

%While the DONN system is employed for ML tasks, such as image classification, phase parameters that modifies the layer-wise diffraction will be optimized through an iterative training process, just like conventional neural networks. However, to precisely model the entire physics phenomenon, unlike conventional DNNs, digital images are represented as complex numbers. With mathematical approximation shown in Section \ref{sec:fourier}, the DONN forward function at numerical level is fully differentiable from detector to laser input. Therefore, the training process of DONNs in LightRidge can be fully integrated with existing automatic differentiation engines and stochastic gradient descent optimization algorithms. To initialize the training process, DONNs w.r.t ML tasks will also have a loss function calculated based on the prediction of the model. Uniquely, DONNs predictions are generated by measuring the output intensity at customized detector regions, which mimics the probabilities of output prediction after \texttt{softmax} in conventional DNNs. For example, mean square error loss (\texttt{MSELoss}) is used in our implementation to guide the training process of DONNs, which is iteratively optimized with training parameters such as training epochs, learning rate, learning rate decaying, etc.

Finally, according to the trained weights and setup parameters, the model is ready to be loaded on the physical hardware. As it is shown in Figure \ref{fig:onn_full}(b), in a 3-layer DONN system for image classification, the input image is encoded with the laser source with wavelength of $532$nm, the diffractive layers are implemented with SLMs, and the detector is implemented with a CMOS camera to generate the final predictions. 
 

\subsection{Fourier Optics and Emulation}
\label{sec:fourier}
 
The DONN system mimics the fully connected neural network in optical domain as shown in Figure \ref{fig:onn_full}(c), and diffraction units in each diffractive layer in the system work as neurons in a fully connected neural network. For the wave propagation in DONN systems, the input wave is described with complex numbers in time domain, and each diffraction unit can be seen as an aperture and a phase modulator, so that the input wave is diffracted and phase-modulated at each diffraction unit.{ Whereas the inference of the physical DONN is all optical, the training part that leads to its design is done through digital computers. }
To make it interpretable for computers, we need mathematical approximation for the wave propagation, i.e., diffraction and phase modulation. 

\subsubsection{Diffraction approximation}
\label{subsec:diff_approx}
 
There are typically three approximation algorithms for scalar theory of diffraction, i.e, \textit{Rayleigh-Sommerfeld approximation}, \textit{Fresnel approximation}, and \textit{Fraunhofer approximation}. They are proposed with different assumptions of the system such as aperture size and propagation distance, and work most efficiently under specific application scenarios. 

The Rayleigh-Sommerfeld is the most commonly used approximation algorithm as it requires least constraints on the system and is reported to give quite accurate results. The Rayleigh-Sommerfeld approximation is implemented with Equation \ref{equ:sommerfeld} in our framework.
\begin{figure}[]
  \centering
  \includegraphics[width=1 \linewidth]{isca2022-latex-template/figs/fourier_img.pdf}
  \caption{Diffraction illustration. \textbf{(a)} ($\xi$, $\eta$) is the plane for diffraction aperture and illuminated by the input light beam in positive $z$ direction, $\Sigma$ on the plane $(\xi, \eta)$ denotes the illuminated area. $(x, y)$ plane is the target plane. $P_{0}$ and $P_{1}$ are illuminated points on two planes. $\theta$ is the angle between the outward normal and the vector pointing from $P_{1}$ to $P_{0}$. \textbf{(b)} Light propagation and phase modulation through the diffractive layer w.r.t the input light wave.}
  \label{figs:diffract_ill}
\end{figure}
As shown in Figure \ref{figs:diffract_ill}, the diffracting aperture is in the $(\xi, \eta)$ plane, and is illuminated in the positive $z$ direction. We calculate the wavefield across the $(x, y)$ plane, which is parallel to the $(\xi, \eta)$ plane and at distance $z$ from it. The $z$ axis pierces both planes at their origins. Then, when $r_{01} \gg \lambda$, the \textit{Rayleigh-Sommerfeld} approximation will be described as
\begin{equation}
\small
    U(x, y) = \frac{z}{j\lambda}\iint \limits_{\Sigma}U(\xi, \eta)\frac{exp(jkr_{01})}{r_{01}^{2}} d{\xi}d{\eta}
\label{equ:sommerfeld}
\end{equation}
where $j=\sqrt{-1}, $ $U(x, y)$ describes the wavefield on target $(x, y)$ plane and $U(\xi, \eta)$ describes the wavefield on the emission $(\xi, \eta)$ plane, $\lambda$ is the wavelength of the input laser, $k$ is the wave number where $k=\frac{2\pi}{\lambda}$, $r_{01}$ is the vector pointing from $P_{0}$ to $P_{1}$ and the distance $r_{01}$ is given by 
\begin{equation}
    r_{01} = \sqrt{z^{2} + (x - \xi)^{2} + (y - \eta)^{2}}
\label{equ:r01}
\end{equation}

When diffraction angle $\theta$ shown in Figure \ref{figs:diffract_ill} is small enough, the computation complexity can be further reduced by applying conditions to the application scenarios while maintaining the emulation accuracy. In \textit{Fresnel approximation}, we further simplify the approximation for the distance $r_{01}$ between $P_{0}$ and $P_{1}$ based on the binomial expansion of the square root in Equation \ref{equ:r01}, where we have
\begin{equation}
    r_{01} \approx z[1 + \frac{1}{2}(\frac{x - \xi}{z})^{2} + \frac{1}{2}(\frac{y - \eta}{z})^{2}]
\end{equation}
The error introduced by dropping all terms but $z$ for $r_{01}$ is generally acceptable for the $r_{01}^{2}$ appearing in the denominator of Equation \ref{equ:sommerfeld} but much more critical for the $r_{01}$ appearing in the exponent. So for $r_{01}$ in the exponent, we retain both terms of binomial approximation. As a result, the Fresnel approximation can be described as
\begin{equation}
    U(x, y) = \frac{e^{jkz}}{j\lambda z} \iint \limits_{\Sigma} U(\xi, \eta)exp\{j\frac{k}{2z}[(x - \xi)^2 + (y - \eta)^2]\}d\xi d\eta
\label{equ:fresnel}
\end{equation}

When we factored the term $exp[\frac{jk}{2z}(x^2 + y^2)]$ out, the Fresnel approximation is expressed as
\begin{equation}
\small
    U(x, y) = \frac{e^{jkz}}{j\lambda z} e^{j\frac{k}{2z}(x^2 + y^2)} \iint \limits_{\Sigma} \{U(\xi, \eta)e^{j\frac{k}{2z}(\xi^{2} + \eta ^ {2})}\}e^{-j\frac{2\pi}{\lambda z}(x\xi + y\eta)} d\xi d\eta
\end{equation}

In Fresnel approximation, the critical approximation happens in the approximation of the exponent, which can be seen that the spherical secondary wavelets will be replaced by wavelets with parabolic wavefronts. Thus, the condition on the distance $z$ will be
\begin{equation}
    z^{3} \gg \frac{\pi}{4\lambda}[(x - \xi)^{2} + (y - \eta)^{2}]^{2}_{max}
\end{equation}
which means the observer (the $(x, y)$ plane) should be in the near field of the aperture. 

The Fraunhofer approximation will greatly simplify the calculations in Fresnel approximation when 
\begin{equation}
    z \gg \frac{k(\xi^{2} + \eta^{2})_{max}}{2}
\end{equation}
is satisfied and quadratic phase factor under the integral sign in Equation \ref{equ:fresnel} is approximately unity over the entire aperture. Thus, in the far field of the aperture, the diffraction can be approximated as 
\begin{equation}
\small
    U(x, y) = \frac{e^{jkz}e^{j\frac{k}{2z}(x^{2} + y^{2})}}{j\lambda z}\iint \limits_{\Sigma} U(\xi, \eta) exp[-j\frac{2\pi}{\lambda z}(x\xi + y\eta)]d\xi d\eta
\label{equ:fraunhofer}
\end{equation}

When an input wave diffracts at the diffractive layers, the input wave will be first transformed to Fourier domain by \textit{Fourier transform} (FFT) and so does the diffraction approximation, those two matrices in Fourier domain will be multiplied to emulate the diffraction. Then, the multiplication result will be transformed back to the time domain by \textit{inverse Fast Fourier Transform} (iFFT) for phase modulation.


\subsubsection{Phase modulation}
 
To realize the modification of the input information in DONN systems, the diffraction unit will apply \textbf{phase modulation} to the input laser beam, which is described with complex numbers. The phase modulation functions like \textit{weight parameters} in conventional neural networks and is updated during training process. Specifically, the input wave can be described by its amplitude and phase, by Euler's formula, it can be described with a complex number in time domain, i.e.,
\begin{equation}
\label{equ:phase_euler}
    m(t) = Ae^{j\theta} = A\text{cos}\theta + jA\text{sin}\theta
\end{equation}
Where $j=\sqrt{-1}$, $A$ is the amplitude, $\theta$ is the phase for the input wave; Acos$\theta$ is the real part and Asin$\theta$ is the imaginary part. When we apply the phase modulation $\phi$, the input wave after phase modulation will be:

\begin{equation}\label{equ:phase_mod}
m(t+1) = Ae^{j(\theta + \phi)} = A\text{cos}(\theta + \phi) + jA\text{sin}(\theta + \phi)
\end{equation}


This function can be realized with a complex number multiplication of the input wave with complex numbers and the phase modulation described with complex numbers, i.e., $P(\phi)$ as shown in Equation \ref{equ:phase_mod_matrix}.

 
\begin{equation} \label{equ:phase_mod_matrix}
\begin{split}
    m(t+1) &= (A\text{cos}\theta + jA\text{sin}\theta) \times (\text{cos}\phi + j\text{sin}\phi)\\
    &= m(t) \times P(\phi)
\end{split}
\end{equation}
 

\iffalse
\begin{equation}
m(t+1) = A \cdot
\left[
  \begin{array}{c}
     \text{cos} \theta\\
     j\text{sin} \theta\\
  \end{array}
\right]^T
\cdot
\begin{bmatrix}
           \text{cos} \phi\\
            j\text{sin} \phi \\
         \end{bmatrix}
\label{equ:phase_mod_matrix}
\end{equation}
\fi

\subsubsection{Measurement of prediction}
\label{sec:measure_pred}
 
To realize the deep learning tasks such as image classifications in physical implementation, we employ the detector at the end of the system which measures the intensity of the light beam. In our simulation, we generate the predictions according to the emulation intensity shown on pre-defined detector regions for different classes. The diffraction and phase modulation are calculated with complex numbers composed of real part and imaginary part, i.e,
\begin{equation}
    E(t) = Re + jIm
\end{equation}
where $E(t)$ describes the light wave at time $t$, $Re$ is the real part and $Im$ is the imaginary part. The intensity $I$ of the light beam would be $I = ({{Re}^{2} + {Im}^{2}})$.  




==> isca2022-latex-template/06sec-physical-verification.tex <==

\section{Validation of LightRidge Physics Engines} \label{sec:validation}
 
As one of the most important objectives of LightRidge compiler is to bridge the gaps between high-level algorithm presentation with low-level physics, verifying the correctness of the physics modeling w.r.t physical optical systems is the first thing for validating the compiler. Specifically, in this section, we perform a sampling-based compiler-physics validation, with the 1) cascaded two-layer diffraction models emulated using LightRidge with CUDA support, and 2) physical two-layer diffraction experimental system (Figure \ref{fig:val}) as the verification bodies.

{\textbf{Input sampling:} Given a cascaded two-layer diffractive model, let the $f$ be the function of the feed-forward diffraction propagation, $f=\text{diffract}(\text{diffract}(x,\text{SLM}_0),\text{SLM}_1)$. Our compiler will take in arbitrary input ($x$) and run the inference with arbitrary phase modulation applied (e.g., $\text{SLM}_0$). Thus, three inputs are sampled in this validation process, i.e., $x$, the full open laser beam; $\text{SLM}_0$, the pattern '7' shown on $\text{SLM}_{0}$; $\text{SLM}_1$, the same pattern '7' as $\text{SLM}_{0}$ shown on $\text{SLM}_{1}$ in Figure \ref{fig:val}. \textbf{Compiler-level measurement:} After the inference with customized input and phase modulation, we will get the intensity distribution over the detector, which will be captured by the \texttt{lr.detector} module. \textbf{Optical system and parameters in compiler}: The wavelength of the laser source is 532nm. Each diffraction unit has the size of 36um $\times$ 36um. For each diffractive layer, we have $40000$ diffraction units which result in a matrix with the size of 200 $\times$ 200. We employ SLMs as the diffractive layers, where the phase modulation of each diffractive unit can be configured externally. Thus, the active physical size of the input and diffractive layers is 7.2mm $\times$ 7.2mm. {\bf Experimental measurement}: To match the propagation of diffraction layers, the active detector region is also set to be 7.2mm $\times$ 7.2mm. Finally, the validation process is conducted by loading the same input and phase modulation, i.e., $x, \text{SLM}_0, \text{SLM}_1$, to LightRidge compiler modeling and the experimental system, and comparing the simulation results of the intensity distribution over the detector plane and the experimental results over the practical detector.} {As we can see from the results in Figure \ref{fig:val}, the features shown in the detection plane in the simulation are verified on the practical detector in the practical hardware system.}


\begin{figure}
     \centering
     \iffalse
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=0.74\textwidth]{isca2022-latex-template/figs/val_7_1.pdf}
         \caption{Validation example 1.}
         \label{fig:val_1}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=0.74\textwidth]{isca2022-latex-template/figs/val_7_2.pdf}
         \caption{Validation example 2.}
         \label{fig:val_2}
     \end{subfigure}
     \fi
     \includegraphics[width=0.5\textwidth]{isca2022-latex-template/figs/new_figure/validation_figures_new-crop.pdf}

     \caption{\color{blue}Experimental validation of LightRidge optical system modules and diffraction engine using a physical cascaded two-layer (SLM$_{0}$ and SLM$_{1}$) diffraction experimental system in visible range. When illuminated by the laser source in an experimental system, the pattern on physical detector is shown in the third figure with red box showing the involved practical detector region. The forth figure shows the emulated pattern at detector with {LightRidge} under the exact setups, which demonstrate the precise correlation between numerical emulation and physical experiments.}
     \label{fig:val}
    % \vspace{-5mm}
\end{figure}



==> isca2022-latex-template/figs/dse_figures.tex <==

\begin{figure*}[t]
     \centering
 
      \begin{subfigure}[b]{0.235\textwidth}
         \centering
    \includegraphics[width=1\textwidth]{isca2022-latex-template/figs/micro22_runtime/runtime_lightridge_cpu-crop.pdf}
         \caption{LightRidge-CPU results.}
        \label{fig:runtime_2}
     \end{subfigure}
    \begin{subfigure}[b]{0.235\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{isca2022-latex-template/figs/micro22_runtime/runtime_lightridge_gpu-crop.pdf}
         \caption{LightRidge-GPU results.}
         \label{fig:runtime_44}
     \end{subfigure}
     \begin{subfigure}[b]{0.235\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{isca2022-latex-template/figs/micro22_runtime/runtime_lightpipe-crop.pdf}
         \caption{LightPipe(2021) results.}
         \label{fig:runtime_1}
     \end{subfigure}
     \begin{subfigure}[b]{0.235\textwidth}
         \centering
         \includegraphics[width=1\textwidth]{isca2022-latex-template/figs/micro22_runtime/cpu_speedups-crop.pdf}
         \caption{CPU speedups.}
         \label{fig:runtime_0}
     \end{subfigure}
     \caption{Runtime evaluation of LightRidge with various workloads of emulating DONNs systems that are configured in different system dimension sizes ($N$) and depths ($D$) -- \textbf{(a)} runtime results collected with LightRidge CPU execution, \textbf{(b)} LightRidge GPU execution, \textbf{(c)} up-to-date LightPipe(2021), and \textbf{(d)} CPU speedups results over LightPipe(2021).}
     \label{fig:runtime}
    % \vspace{-5mm}
\end{figure*}


==> sec-compiler-old.tex <==
\section{LightRidge Compiler}\label{sec:overview}

%{\color{red} paragraph will be expanded to subsections later.}

\begin{figure}[t]
  \centering
  \includegraphics[width=1 \linewidth]{isca2022-latex-template/figs/new_figure/compiler_system_overview_new.pdf}
  \caption{\color{blue}Overview of LightRidge compilation stack, including design, emulation, training, and deployment.}
  \label{figs:overview}
\end{figure}


{In this section, we describe the programming modules implemented in LightRidge. Our framework (Figure \ref{figs:overview}) aims to simplify and accelerate the process of design, exploration and deployment of the DONNs, such that it consists of \textbf{a)} versatile programming modules for user-defined optical systems, \textbf{b)} optical laser modules, \textbf{c)} physics modeling of diffraction, \textbf{d)} system measurement modeling under optical meaning, \textbf{e)} DONN architecture construction and physics-aware training, and \textbf{f)} hardware deployment. 


Each component can be customized as simple as entering specific parameters like wavelength for laser source, aperture size, approximation algorithms for diffraction modeling, detector design for measurement, selection of training algorithms, etc. In the rest of this section, we illustrate the programming capability of LightRidge by introducing the modules for each component of DONNs, including optical system setup, DONN construction, training, and deployment.} %To construct a simple feed-forward DONNs architecture, diffractive layers and detector can be stacked together and are fully differentiable. %To take advantages of Pytorch and existing machine learning algorithms, we design each module as differentiable and models can be trained easily with existing training engines for conventional neural networks, e.g., \texttt{Adam} for optimization.




\subsection{Global system definitions}  
\label{subsec:user_param}
%Unlike the compilation of conventional neural networks, the design, training, and deployment process of DONNs are highly sensitive to the physical optical setups, which are mostly determined by the application scenarios. 
DONN design and architecture are determined to the wavelength/frequency of the light that encodes the input features. {To initialize the compilation process of a DONN system w.r.t specific physical optical systems, the DONN architecture requires the following configurations supported by LightRidge -- (1) the laser profile such as wavelength/frequency and beam profile globally impacts the design, architecture exploration, and deployment of DONNs, (2) architecture configurations such as diffraction pixel size to be fabricated, number of diffraction units, DONNs depths, etc., need to carefully be configured for different ML tasks, (3) and the training and validation parameters of DONNs before and at the deployment stage. 

For example, as shown in Listing \ref{code:user_para}, depending on the laser source we have at hand, {the \texttt{wavelength} of the laser source will be set as 532nm, and the \texttt{laser profile} is set to be a Gaussian beam. Decided by the laser wavelength, we set the size of the diffraction unit in the layers (\texttt{unit\_size}) as 36$\text{um} \times$ 36um and the \texttt{distance} between source to diffractive layer, layers to layers, and layer to the detector is set to be 28cm}. The distance between each component can also be adjusted according to the requirements. %We are going to employ the proposed DONN system to realize the image classification with MNIST dataset (\texttt{dataset}). 
Training parameters are also initialized at this stage. As shown in this example, the training \texttt{Adam} optimizer \cite{kingma2014adam} implemented in PyTorch is set to be the optimizer with learning rate \texttt{lr} of 0.5. We will discuss how PyTorch optimizer can be leveraged directly to the DONN training process in Section \ref{subsec:phy_model}.}

%The parameters are provided for two parts -- (1) one for the customized optical system like wavelength for laser source and number of layers in the model; (2) the other one for the deep learning task with the DONN model like which dataset will be implemented and what optimization algorithm will be employed. For example, as shown in Listing \ref{code:user_para}, depending on the laser source we have at hand, {\color{red}the \texttt{wavelength} of the laser source will be set as 0.75mm, which lies in THz range, and the \texttt{laser profile} is set to be a Gaussian beam. Decided by the laser wavelength, we set the size of the diffraction unit in the layers (\texttt{unit\_size}) as 0.4$\text{mm} \times$ 0.4mm and the \texttt{distance} between source to diffractive layer, layers to layers, and layer to the detector is set to be 0.08m}. The distance between each component can also be adjusted according to the requirements. We are going to employ the proposed DONN system to realize the image classification with MNIST dataset (\texttt{dataset}). We set the \texttt{optimizer} as \texttt{Adam} with learning rate (\texttt{lr}) of 0.5. All the parameters proposed by users are taken into LightRidge to initialize the DONN model and its training.   

\begin{lstlisting}[language=Python, caption={Global definitions and system constraints of DONNs.}, label=code:user_para]
# define user parameters
# for laser source
lr.laser_profile.wavelength = 532e-9
lr.laser_profile.src_profile = 'Gaussian'
lr.laser_profile.waist = 2.9e-4
lr.laser_profile.aperture_radius = 2e-5
lr.laser_profile.aperture_dist = 2e-3
# for DONN systems
lr.diffraction.unit_size = 0.000036
lr.diffraction.distance = 0.28
lr.diffraction.sys_size = 200
depth = 5
lr.laser_profile.init()
lr.diffraction.init()
# for training
lr.model.train(optimizer = torch.optim.adam, lr = 0.5, batch_size = 500, epochs = 10)
\end{lstlisting}

\subsection{Laser profile} 
%\label{subsec:laser}
%With parameters provided and the python package LightRidge imported (import \texttt{lightRidge} as \texttt{lr}), components in an DONN model are ready to be customized. 
The first part of our framework is the design for the laser source in \texttt{lr.laser}, which will precisely offer conventional laser profiles that include laser specifications such as \texttt{wavelength}, \texttt{aperture}, etc. For example, we have implemented a widely used Gaussian beam profile taking the defined waist and two apertures, i.e., ring aperture and rectangle aperture, for applications. %For example, to implement a laser source with a Gaussian beam, we can call the block in the compiler by executing the single code \texttt{lr.laser.GaussBeam} and define its wavelength, aperture, and waist inside the block. 
Note that laser profile building block is critical to compiling any DONNs, since these parameters will be passed to all other building blocks discussed later. 

%Wavelength is a user-defined parameter for laser source. Currently, two apertures, ring aperture and rectangle aperture, are implemented in LightRidge. The profile for laser such as Gaussian profile can be implemented with \texttt{lr.laser.GaussBeam}. %With more characteristics of the laser source implemented in the simulation, users will get better consistency between numerical modeling and deployment.

\iffalse
\begin{lstlisting}[language=Python, caption= Customization of the laser source , label=code:laser_src]
import LightRidge as lr
# define laser source information
# aperture
aperture = RingAperture(radius, sys_size, aperture_dist, pixel_size=3.6e-5)
# profile
GaussMask = lr.laser.GaussBeam(waist=waist,size=size)
# input laser to the system
x_train = torch.square(torch.abs(
                    aperture(GaussMask(x_train)))
\end{lstlisting}
\fi

\subsection{Physics modelling of diffraction} 
\label{subsec:phy_model}

In the DONN system, phase modulations include trainable parameters, which realize data movements by light diffraction. %The input light wave and phase modulation will be both described with complex numbers. 
The main concept of DONNs in learning complex ML tasks is stacking such phase modulation and diffraction like conventional neural network layers, and optimize the phase parameters similarly as the conventional weight parameters. Thus, we introduce layer-wise physical modelling for diffraction and phase modulation with building block \texttt{lr.layers}. The algorithm for approximating the diffraction in the free-space system will be defined based on the laser source. Specifically, according to what we have discussed in Section \ref{subsec:diff_approx}, three major approximation algorithms in diffraction are implemented in our framework -- (1) \textit{Rayleigh-Sommerfeld Approximation}, implemented with Equation \ref{equ:sommerfeld}, which is the most accurate approximation algorithm but also a most complex one; (2) \textit{Fresnel Approximation}, implemented with Equation \ref{equ:fresnel}, which is an approximation for the propagation with parabolic wavefronts, namely the near field propagation; (3) \textit{Fraunhofer Approximation}, implemented with Equation \ref{equ:fraunhofer}, an approximation for the propagation with planar wavefronts, which is used to approximate the far field propagation \cite{tobin1997introduction}. Approximation algorithms can be selected by one of the following keywords, i.e., \texttt{Sommerfeld}, \texttt{Fresnel}, \texttt{Fraunhofer}, to the argument \texttt{approx} in the module \texttt{lr.layers.DiffractLayer}.
%Our system will take Rayleigh-Sommerfeld approximation as default.

The phase modulation encoded on the diffractive layers will be applied to the light wave by matrix multiplication as shown in Equation \ref{equ:phase_mod_matrix}. Specifically, when the input light wave projects on a diffractive layer, the input wave field is first transformed to Fourier domain by \textit{Fast Fourier Transform} (FFT) and matrix-multiplied with the {specific approximation functions selected} by the keyword \texttt{approx}. Then, the result matrix will be transformed to the time domain by \textit{inverse Fast Fourier Transforms} (iFFT) for phase modulation, where the matrix will be multiplied with another trainable matrix representing the phase changes.

The approximation functions are the most computation-intense cores in the compiler. Specifically, the forward function of diffraction requires FFT, iFFT, and complex matrix multiplications, which can take advantages of modern CPU and GPU platforms. {In addition, similarly to the front-end compilers of conventional neural networks, batched operations are critical in training, inference, and exploration runtime efficiency. Thus, LightRidge physics engine is designed to elaborate the conventional front-end ML compilers to improve runtime. Specifically, we develop the three diffraction approximations using PyTorch accelerated Fast Fourier Transforms modules. To enable batched operations on DONNs simulation, two-dimensional FFT and iFFT are deployed with batched complex tensors as inputs, which encode the input laser source or diffraction output from the previous layer. Complex matrix multiplications are mimicked with two parallel matrix multiplications. Unlike the state-of-the-art optics simulation framework LightPipe \cite{vdovin1997lightpipes}, the runtime of diffraction model simulation in LightRidge will natively support Intel’s MKL-FFT library \cite{wang2014intel} on Intel CPUs, and Nvidia’s cuFFT library \cite{podlozhnyuk2007fft} on CUDA devices, which have been carefully optimized in PyTorch. \textbf{Results in Section \ref{sec:runtime_result} show that our framework demonstrates up to 105$\times$ speedups on CPU, and up to 7,661$\times$ on CUDA devices, compared to LightPipe.} Detailed runtime comparisons are provided in Section \ref{sec:runtime_result}}.

%{\color{red}Additionally, to improve the accuracy performance of DONN systems with few diffractive layers ($\leq$ 3 layers), we introduce a hyperparameter \texttt{reg\_factor} in the simulation to regularize the gradients generated in the training process for DONN systems. The results in Section \ref{sec:evaluation} show our compiler with regularization will improve the simulation accuracy significantly for less complex DONNs. }
%For example, for the system with 1 diffractive layer, the simulation with LightRidge can get an accuracy of $0.98$ by setting the regularization factor as $90$ and it is $37\%$ increase compared to that in \cite{lin2018all} without regularization. For the system with 3 diffractive layers, the accuracy will increase from $0.91$ to $0.98$ with our compiler. 

\iffalse

\begin{lstlisting}[language=Python, caption=Example code blocks of diffractive layer modeling., label=code:phys_model]
import LightRidge as lr
# define the diffractive layer
lr.laser_profile.init()
lr.diffraction.init()
l1 = lr.layers.DiffractLayer(sys_size, pixel_size, approx='fresnel', ...)
l2 = lr.layers.DiffractLayer(sys_size, pixel_size, approx='fresnel', ...)
...
# Note: approx = 'sommerfeld' or 'fraunhofer' will select the other two approximation functions
\end{lstlisting}
\fi
%\cunxi{needs to show exact kernel implementation of all three approximations in PYTHON}

%\paragraph{\cunxi Kernel implementation basics}

%FFT IFFT Complex multiplication

%\paragraph{\cunxi Sommerfeld} h=?

%\paragraph{\cunxi Fresnel} h=?

%\paragraph{\cunxi Fraunhofer} h=?


%Another important component in the DONN system is the detector, which will capture the light intensity after diffraction and phase modulation. By analysing the intensity distribution on the detector with the pre-defined detector regions for different labels, we can get the final predication. LightRidge provides customization for detectors in \texttt{lr.layers.Detector}. Arbitrary observing pattern on detector plane can be designed with coordinates of the top-left corner of detector regions and the detector size provided. In our framework, the shape of each detector region is set to be square by default.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9 \linewidth]{isca2022-latex-template/figs/detector_api.pdf}
  \caption{Illustration example of the detector measurement enabled by \texttt{lr.layers.Detector} for a 10-class classification DONNs system. %, with the \texttt{x\_loc} and \texttt{y\_loc} arguments indicate the locations of the detector region for measuring the intensity for classification. %Note that activation function is only used for training the physical parameters in LightRidge, where physical measurement is performed directly with \texttt{argmax} on detector.
  }
 % \vspace{-3mm}
  \label{figs:detector}
\end{figure}

\subsection{Detector design}
 
{To convert the final outputs of DONNs into predictions (e.g., classification results), frequency-specific detectors are required to capture the intensity value of resulting light coming from the multi-layer diffraction and phase modulation. Specifically, by measuring the intensity distribution at the detector plane, carefully designed detector regions are important user-specific DONN architecture parameters. For example, for multi-label image classification tasks with $N$ classes, $N$ pre-defined detector regions will be specified that collect the intensity values of the light in each region, which is used for generating the final prediction using \texttt{argmax} just like conventional DNNs. %In other words, detector can be considered as the final layer for prediction in conventional neural networks. 
%Note that these pre-defined detector regions require domain-specific customization in different detectors and different laser profile. 
Thus, LightRidge provides customization for detectors via the compiler module \texttt{lr.layers.Detector}, which includes three major arguments: \textbf{(1)} 2D coordinates of the detector regions \texttt{x\_loc} and \texttt{y\_loc}, where the inputs are $N$ element lists, \textbf{(2)} detector size \texttt{det\_size}, which is the unit element in measuring the light intensity at the detector; \textbf{(3)} activation function used for training \texttt{activation}.} {We illustrate the Detector module in our framework using Figure \ref{figs:detector}, which construct a detector design for 10-class classification problem. %Note that the output of diffraction is in the complex-domain that contains both amplitude and phase information of the light, while the optical detector mostly measures the intensity of the light. Thus, to make final predictions in both emulation and experiments, the transformation from complex numbers to detectable intensity will be realized with the algorithm shown in Section \ref{sec:measure_pred}. During the training process, the light intensity over ten pre-defined detector regions, i.e., a $1 \times 10$ vector, read from the detector will first be applied with an activation function, which is \texttt{softmax} in this illustration, before \texttt{argmax} is applied for the final prediction. 
%While in the inference, \texttt{argmax} will be applied directly to the light intensity vector read from the detector, to incorporate with the physical optical detector that is very challenging to add nonlinearity.
}

\iffalse
\begin{lstlisting}[language=Python, caption={Detector design example in LightRidge.~Note that activation function is only used in training. Physical optical detector generates final prediction with \texttt{argmax}.}, label=code:det]
# Detector design, system size would be 200x200, ten classes in total, detector size would be 10x10
lr.layers.Detector(x_loc=[], y_loc=[], det_size, activation=torch.nn.functional.softmax, mode='intensity')
# mode = 'intensity' or 'amplitude' or 'phase' for analyzing other properties of the light output
\end{lstlisting}
\fi

 
\subsection{Diffractive neural architecture construction}

%With all components setup well, the DONN model will be simply constructed customized by setting a \texttt{class} model with all components imported. During model construction, LightRidge allows stacking arbitrary number of diffractive layers and placing layers at designed positions by adjusting the argument \texttt{distance}.

{As shown in Listing \ref{code:model_const}, with aforementioned fundamental optical modules, the DONN model can be simply constructed by stacking the diffractive layers modules implemented in \texttt{lr.layers}). Similar to conventional DNNs, the neural architecture of DONNs is a multi-layer feed-forward function consisting of a series of diffraction and phase modulation. Thus, to construct a DONNs model, LightRidge allows stacking arbitrary numbers of diffractive layers w.r.t designed physical optical system parameters, such as layer to layer distance, number of diffractive units, physical dimensions, per layer hardware parameters, etc. This DONNs \texttt{class} can be treated as a sequential container, where diffractive layer modules will be added to it in the order they are passed in and “chains” outputs to inputs sequentially for each subsequent module, finally returning the output of the last module.}

As a result, LightRidge compiler provides great flexibility for customizing the DONN model enabled by the versatile fundamental optical physics modeling. Here, we emphasize the following major versatile factors: 1) as discussed in Section \ref{sec:donn}, there is wide range of laser frequency that can be used; 2) heterogeneous design can be realized by defining different diffractive layers in the DONN system. Specifically, our compiler supports separate definitions for each diffractive layer. For example, the distance between the first and the second layer can be different from that between the second and the third layer by adjusting different \textit{distance} hyperparameters when implementing the second and the third layer.

\begin{lstlisting}[language=Python, caption=Model construction and CUDA acceleration of optical physics emulation examples., label=code:model_const]
###Model construction
# User-defined model composed based on components defined in 
# Physical Modelling and Detector Setup
class Model(torch.nn.Module):
    # initial arguments definition for the model
  def __init__(...)
        ...
    self.diffractive_layers_1=l1
    self.diffractive_layers_2=l2
        ...
    self.last_diffraction=layers.DiffractiveLayer(..., phase_mode = False)
    self.detector = lr.layers.Detector(...)
  def forward(self, x):
    x = self.diffractive_layers_1(x)
    x = self.diffractive_layers_2(x)
    ...
    x = self.last_diffraction(x)
    output = self.detector(x)
    return output

# emulation and training will be executed on Nvidia GPU.
model = Model(...).to("cuda")
\end{lstlisting}


\subsection{Training modules}

%{One of the critical components in LightRidge is to enable efficient physics-aware training of DONNs. For most of the conventional compilers for efficient hardware deployment, the compilation and optimizations are designed to enable efficient deployment of post-training models and automates optimization of low-level programs to hardware characteristics. Therefore, the training mechanisms of conventional neural networks are mostly supported by front-end ML compilers such as PyTorch, Tensorflow, etc. Note that training algorithms of conventional neural networks have been very well developed and can be easily extended and integrated in many other optimization tasks. For example, PyTorch optimizer module \texttt{torch.optim} implements various efficient optimization algorithms and has been highly optimized in performance and runtime. As most commonly used methods are already supported, and the interface is general enough, LightRidge training modules are built around the existing gradient descent optimization algorithms.}

%Most commonly used methods are already supported, and the interface is general enough, so that more sophisticated ones can be also easily integrated in the future.
 
%Then, machine learning task will be specified w.r.t the DONN model. For DONN model, the input information will be encoded on the laser beam. In optical domain, light will be described with complex numbers which involve real part and imaginary part. With the complex number description, we can get both amplitude and phase information of the information-carried light beam. In our framework, inputs will first be converted to complex domain by \texttt{lr.utils.data\_to\_cplex()}. At the output/detector plane, the intensity will be measured as the network output and compared with the ground truth label in the loss function, e.g., \texttt{MSELoss} for the loss function. With all components implemented as differentiable modules, the DONN model is fully differentiable, such that it can be trained with conventional automatic differentiation engine, e.g., \texttt{Adam} for optimization. 


Here, we introduce the training/optimization modules in LightRidge by focusing on ML tasks, particularly image classification problems, which natively supports PyTorch automatic differentiation (\texttt{autograd}) mechanism. For DONN model, the input information will be encoded on the laser beam. In optical domain, light will be described with complex numbers which involve real part and imaginary part. With the complex number description, we can get both amplitude and phase information of the information-carried light beam. In our framework, inputs will first be converted to complex domain by \texttt{lr.utils.data\_to\_cplex()}. At the output/detector plane, the intensity will be measured as the network output and compared with the ground truth label in the loss function, e.g., \texttt{MSELoss} for the loss function. With all components implemented as differentiable modules, the DONN model is fully differentiable, such that it can be trained with conventional automatic differentiation engine, e.g., \texttt{Adam} for optimization. 

As a result, in the forward function, the DONNs model makes its prediction based on the diffraction propagation and the prediction of the given feature is then made at the detector plane. In other words, it runs the input data through every diffraction and phase modulation to make its prediction. During the backpropagation phase, the DONNs will adjust its \textbf{phase modulation parameters} proportionate to the error made in the forward function. Note that the phase modulation parameters correspond to specific physical parameters (e.g., thickness of materials) or supplying voltage value on devices (e.g., SLMs and phase change material). Similarly, this is done by traversing backward from the output, collecting the derivatives of the error with respect to the parameters of diffraction functions (i.e., FFT, IFFT, and complex-domain matrix multiplication), and optimizing the parameters using gradient descent algorithms.


\iffalse

\begin{lstlisting}[language=Python, caption=Model training. The inputs will first be converted to complex domain. Conventional optimization engines can be employed in the training., label=code:training]
# Training/ Testing setup
# Convert original gray-scale images into complex domain
x_train, y_train = lr.utils.data_to_cplex(train_loader)
x_test, y_test = lr.utils.data_to_cplex(test_loader)
# Apply laser mask to input images
x_train = torch.square(torch.abs(aperture(GaussMask(x_train)))
# Define loss criterion, optimization algorithm, etc. 
def train():
  ...
  optimizer = torch.optim.Adam(model.parameters(), lr=lr)
  criterion = torch.nn.MSELoss(reduction='sum')
  train_loss_ = criterion(train_outputs, train_labels)
\end{lstlisting}

\fi


\iffalse
\begin{lstlisting}[language=Python, caption=Back-end deployment support and propagation measurement., label=code:model_backend]
# simulation visualization
# view phase modulation
model.phase_view()
# view propagation 
model.prop_view()
# Generate phase mask with 3D printer
model.to_3d_render(3d_print_specs)
# Generate phase mask with SLM
model.to_slm(slm_specs)
\end{lstlisting}
\fi

%The code in our system is designed based on \texttt{pytorch}. Taking advantage of GPU and \texttt{pytorch}, we modulate the design components, simplifying the process of designing diffractive optical neural network. With our system, users can simulate their designed diffractive models easily and the design efficiency can be improved greatly.


\subsection{Complex-domain Regularization}
\label{sec:regu}

In our implementation, considering the physics in optics, the DONN system is described and emulated with complex numbers. According to \cite{lin2018all} and Equation \ref{equ:phase_mod_matrix}, the training for DONN system is more phase modulation dominated and the intensity at the end of diffraction will decrease exponentially as the number of diffractive layers increases, which means a regularization between amplitude and phase is required to avoid gradient vanishing and explosion in training process. Thus, we introduce a novel regularization factor $\lambda$ in the forward function described in {Equation \ref{equ:phase_mod_matrix}} to improve the training efficiency, which can flexibly change the gradient scales between amplitude and phase modulations. Specifically, $\lambda$ is applied to amplitude vector $A$ in Equation \ref{equ:phase_euler}. 
%Let $\mathcal{M}$ as the mapping of $(w^{i, j}, A, P) \xrightarrow{\mathcal{M}} w^{i,j}_{\mathbb{C}}$. Let $\nabla w^{i,j}_{\mathbb{C}}$ be the upstream gradient to calculate $\nabla w^{i,j}$. The difference of the gradient updates can be summarized as follows: 
\iffalse
\begin{equation*}
\begin{split}
   \nabla w^{i,j} = {\nabla w^{i,j}_{\mathbb{C}}} \cdot \frac{ \frac{\partial \mathcal{M}}{\partial{w^{i, j}}} \cdot A + \frac{\partial \mathcal{M}}{{\partial{w^{i, j}}}} \cdot P}{2} ~~~~ \xRightarrow{~~~~\lambda~~~~} ~~~~ \\
   \nabla w^{i,j}_{reg} = \nabla w^{i,j}_{\mathbb{C}} \cdot \frac{ \frac{1}{\lambda} \cdot ( {\frac{\partial{\mathcal{M}}}{\partial{w^{i, j}}} \cdot {A}}) + \frac{\partial{\mathcal{M}}}{\partial{w_{i, j}}} \cdot P}{2}
\end{split}
    \label{equ:grad}
\end{equation*}
\fi
%The gradients will be backpropagated as shown in Equation \ref{equ:grad}. 
%Since in DONNs system, the intensity of the input light decreases exponentially as the diffractive layers increase, the amplitude used in our system will decrease exponentially as expected. For the two integrated parameters, phase and amplitude, controlled by one device discrete state, amplitude will change with the depth implemented in the system while phase will not. Thus, the regularization factor $\lambda$ is introduced to avoid gradient explosion and vanishing, which compensates the effects caused by the change of system depth. According to Equations \ref{equ:grad}, this regularization factor adjusts the weight of upstream gradients calculated on the amplitude and phase. 

Since in DONN system, the intensity of the input light decreases exponentially as diffractive layers increase, the weight of amplitude modulation in forward and backward propagation are expected to decrease exponentially, as the number of layers increases. Thus, the optimal value for the algorithmic parameter $\lambda$ needs to be explored for different DONNs architectures. Empirically, $\lambda$ should be $\geq$1, i.e., compensating the loss for the intensity after propagating through each diffractive layer. %In Section \ref{subsec:conf_test}, we explore the performance of the proposed regularization technique with 1, 3 and 5 diffractive layers in DONNs, which confirms the discussed regularization characteristic.
%Moreover, as the results in section \ref{sec:result_regu} show, even though systems with different diffractive layers can all be trained to acquire a decent accuracy performance with no much difference by adjusting the regularization factor in training process, the classification confidence can vary significantly. As diffractive layers increase in the system, the classification problem can be finely tuned and explored with more neurons involved. Thus, the predictions will be more confident. 

\subsection{Hardware deployment and visualization}
Users can view the phase modulation for each diffractive layer by executing \texttt{model.phase\_view} and view the propagation process by executing \texttt{model.prop\_view}. More importantly, the proposed compiler directly supports various popular hardware deployment w.r.t to specific laser source. Specifically, LightRidge supports different fabrication/deployment methods, e.g., SLMs for laser in visible range and 3D printed phase mask for THz systems. Our framework can directly interface with these two types of hardware backends, e.g., \texttt{model.to\_slm} for EXULUS-HD1 SLMs and \texttt{model.to\_3d\_render} for FormLab 3D printers.
